Generalized Lineage-Aware Temporal Windows: Supporting Outer and Anti Joins in Temporal-Probabilistic Databases

The result of a temporal-probabilistic (TP) join with negation includes, at each time point, the probability with which a tuple of a positive relation ${\bf p}$ matches none of the tuples in a negative relation ${\bf n}$, for a given join condition $\theta$. TP outer and anti joins thus resemble the characteristics of relational outer and anti joins also in the case when there exist time points at which input tuples from ${\bf p}$ have non-zero probabilities to be $true$ and input tuples from ${\bf n}$ have non-zero probabilities to be $false$, respectively. For the computation of TP joins with negation, we introduce generalized lineage-aware temporal windows, a mechanism that binds an output interval to the lineages of all the matching valid tuples of each input relation. We group the windows of two TP relations into three disjoint sets based on the way attributes, lineage expressions and intervals are produced. We compute all windows in an incremental manner, and we show that pipelined computations allow for the direct integration of our approach into PostgreSQL. We thereby alleviate the prevalent redundancies in the interval computations of existing approaches, which is proven by an extensive experimental evaluation with real-world datasets.

==> 4a_properties_fig.tex <==
\begin{figure*}[ht]\centering
\setlength{\tabcolsep}{5pt}
\def\arraystretch{1.2}
\begin{subfigure}[b]{0.2\linewidth} \centering
\scalebox{0.82}{
\begin{tabular}{c|c|c|c}
\multicolumn{4}{l}{$\mathbf{a}$ \textbf{(productsBought)}} \\
\hline
\textit{$F_r$}  & $\lambda$ & $T$ & $p$ \\ \hline
\bsq{a} & $a_1$ & {[2,10)} & {0.3} \\
\bsq{b} & $a_2$ & {[4,7)}  & {0.8} \\
\bsq{c} & $a_3$ & {[5,9)}  & {0.7} \\ 
\end{tabular}}
\vspace*{0.2cm}

\scalebox{0.82}{
\begin{tabular}{c|c|c|c}
\multicolumn{4}{l}{$\mathbf{b}$ \textbf{(productsOrdered)}}\\
\hline
\textit{$F_s$} & $\lambda$ & $T$ & $p$ \\ \hline
\bsq{a} & $b_1$ & {[3,7)}  & {0.6} \\
\bsq{a} & $b_2$ & {[8,12)} & {0.6} \\
\bsq{b} & $b_3$ & {[5,8)}  & {0.7} \\ \hline
\end{tabular}}
\caption{Input Relations}
\label{fig:propertiesInput}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{minipage}[b]{0.57\linewidth}
\begin{subfigure}[b]{0.78\linewidth} \centering
\scalebox{0.82}{
\begin{tabular}{c|c|c|c}
\multicolumn{4}{l}{Q = $\bf a \ -^\kat{Tp} \ \ b$}\\
\hline 
\textit{F} & $\lambda$ & $T$ & $p$ \\ \hline
\bsq{a} & $a_1$ & {[2,3)}  & {0.3} \\
\bsq{a} & $a_1 \land \lnot b_1$ & {[3,7)}  & {0.3} \\
\bsq{a} & $a_1 \land \lnot b_2$ & {[8,10)}  & {0.3} \\
\bsq{b} & $a_2$ & {[4,5)}  & {0.7} \\ 
\bsq{b} & $a_2 \land \lnot b_3$ & {[5,7)}  & {0.3} \\
\bsq{c} & $a_3$ & {[5,9)}  & {0.3} \\ \hline
\end{tabular}}
\qquad
\scalebox{0.82}{
\begin{tabular}{c c|c|c|c}
\multicolumn{4}{l}{Q = $\bf b \ \bowtie_\theta^\kat{Tp} \ \ a$,
\ $\theta: F_r > F_b$}\\
\hline 
\textit{F$_r$} & \textit{F$_s$} & $\lambda$ & $T$ & $p$ \\ \hline
\bsq{a} & \bsq{b} & $b_1 \land a_2$ & {[4,7)}  & {0.3} \\
\bsq{a} & \bsq{c} & $b_1 \land a_3$ & {[5,7)}  & {0.3} \\
\bsq{b} & \bsq{c} & $b_3 \land a_3$ & {[5,8)}  & {0.3} \\
\end{tabular}}
\qquad
\scalebox{0.82}{
\begin{tabular}{c c|c|c|c}
\multicolumn{4}{l}{Q = $\bf a \ \RJoin_\theta^\kat{Tp} \ \ b$,
\ $\theta: F_r > F_b$}\\
\hline 
\textit{F$_r$} & \textit{F$_s$} & $\lambda$ & $T$ & $p$ \\ \hline
\bsq{a} & \bsq{b} & $b_1 \land a_2$ & {[4,7)}  & {0.3} \\
\bsq{a} & \bsq{c} & $b_1 \land a_3$ & {[5,8)}  & {0.3} \\
\bsq{a} & -       & $b_2$ & {[8,12)}  & {0.3} \\
\bsq{b} & \bsq{c} & $b_3 \land a_3$ & {[5,8)}  & {0.3} \\
\bsq{a} & -       & $b_1 \land \lnot a_2$ & {[4,5)}  & {0.3} \\
\bsq{a} & -       & $b_1 \land \lnot (a_2 \lor a_3)$ & {[5,7)} & 0.3\\
\bsq{a} & -       & $b_1 \land \lnot a_3$ & {[7,8)}  & {0.3} \\
\end{tabular}}
%%%%%%%%%%%%%%%%%
\caption{Query Result}
\label{fig:propertiesResults}
\end{subfigure}
%\end{minipage}
\caption{Property illustration}
\label{fig:propertiesExample}
\end{figure*}

==> 6_algebra_definitions.tex <==
In this section, we express the results of TP outer joins and TP
anti join using the generalized lineage-aware temporal windows
produced for two input relations and a predicate. Each generalized 
lineage-aware temporal window $w = (F_r, F_s, T, \lambda_r,
\lambda_s)$ corresponds to exactly one output tuple. 



\begin{definition} \label{def:tpJoins} {\it (TP Joins)}
  {\em Let ${\bf r}$ and ${\bf s}$ be tem\-poral-probabilistic
    relations with schema ($F$, $\lambda$, $T$, $p$). Given the
    lineage-concatenation functions depicted in 
    Table~\ref{tab:lineageFunctions}, we define the join
    operations 
%    $\mathbf{r} \times^\kat{Tp} \mathbf{s}$,
%    $\mathbf{r} \bowtie_{\theta}^\kat{Tp} \mathbf{s}$,
    $\mathbf{r} \LJoin_{\theta}^\kat{Tp} \mathbf{s}$,
    $\mathbf{r} \RJoin_{\theta}^\kat{Tp}
    \mathbf{s}$, $\mathbf{r} \AJoin_{\theta}^\kat{Tp} \mathbf{s}$
    and $\mathbf{r} \OJoin^\kat{Tp} \mathbf{s}$ as follows:}
   
\begin{table}[h] \centering 
  \fontsize{9pt}{11pt}\selectfont
  \setlength{\tabcolsep}{2pt}
    \begin{tabular}{M{1.7cm} M{0.8cm} l}
      \hline
%%%%%%%%%%%%%%%%%%%%%%%  LEFT JOIN  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{\noindent $\tilde{r}\ \in \mathbf{r} \ 
\LJoin_{\theta}^\kat{Tp} \ \mathbf{s}$}
&  \multirow{4}{*}{$\Longleftrightarrow$}
%& $\pi_\kat{$F_r$,\ $F_s$, T,\ $\lambda_r / \lambda$}
%   (W_{\kat{UF}}({\bf r}; {\bf s}, \theta))$ \ $\cup$ \\
%&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  $\lambda_r / \lambda$}
  ({\bf W_\kat{U}}({\bf r}; {\bf s}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  and$(\lambda_r,\lambda_s) / \lambda$}
  ({\bf W_{\kat{O}}}({\bf r}; {\bf s}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  andNot$(\lambda_r,\lambda_s) / \lambda$}
  ({\bf W_\kat{N}}({\bf r}; {\bf s}, \theta))$
  \\ [0.5ex]
\hline
%%%%%%%%%%%%%%%%%%%%%%%  RIGHT JOIN  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{4}{*}{\noindent $\tilde{r}\ \in \mathbf{r} \ \RJoin_{\theta}^\kat{Tp} \ \mathbf{s}$}
&  \multirow{4}{*}{$\Longleftrightarrow$}
%& $\pi_\kat{$F_r$,\ $F_s$, T,\ $\lambda_r / \lambda$}
%   (W_{\kat{UF}}({\bf s}; {\bf r}, \theta))$ \ $\cup$ \\
%&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  $\lambda_r / \lambda$}
  ({\bf W_\kat{U}}({\bf s}; {\bf r}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  and$(\lambda_r,\lambda_s) / \lambda$}
  ({\bf W_{\kat{O}}}({\bf s}; {\bf r}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  andNot$(\lambda_r,\lambda_s) / \lambda$}
  ({\bf W_\kat{N}}({\bf s}; {\bf r}, \theta))$
  \\ [0.5ex]
\hline
%%%%%%%%%%%%%%%%%%%%%%%  ANTI JOIN  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{3}{*}{\noindent $\tilde{r}\ \in \mathbf{r} \AJoin_{\theta}^\kat{Tp} \mathbf{s}$}
&  \multirow{3}{*}{$\Longleftrightarrow$}
%& $\pi_\kat{$F_r$,\ $F_s$, T,\ $\lambda_r / \lambda$}
%   (W_{\kat{UF}}({\bf r}; {\bf s}, \theta))$ \ $\cup$ \\
%&
& $\pi_\kat{$F_r$, T,\
  $\lambda_r / \lambda$}
  ({\bf W_\kat{U}}({\bf r}; {\bf s}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
& $\pi_\kat{$F_r$, T,\
  andNot$(\lambda_r,\lambda_s) / \lambda$}
  ({\bf W_\kat{N}}({\bf r}; {\bf s}, \theta))$
  \\ [0.5ex]
\hline
%%%%%%%%%%%%%%%%%%%%%%%  FULL JOIN  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{ 2}{*}{\noindent $\tilde{r}\ \in \mathbf{r} \OJoin_{\theta}^\kat{Tp} \mathbf{s}$}
&  \multirow{ 2}{*}{$\Longleftrightarrow$}
%& $\pi_\kat{$F_r$,\ $F_s$, T,\ $\lambda_r / \lambda$}
%   (W_{\kat{UF}}({\bf r}; {\bf s}, \theta))$ \ $\cup$ \\
%&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  $\lambda_r / \lambda$}
  ({\bf W_\kat{U}}({\bf r}; {\bf s}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  and$(\lambda_r,\lambda_s) / \lambda$}
  ({\bf W_{\kat{O}}}({\bf r}; {\bf s}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
& $\pi_\kat{$F_r$,\ $F_s$, T,\
  andNot$(\lambda_r,\lambda_s) / \lambda$}
  ({\bf W_\kat{N}}({\bf r}; {\bf s}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
%& $\pi_\kat{$F_r$,\ $F_s$, T,\ $\lambda_r / \lambda$}
%   (W_{\kat{UF}}({\bf s}; {\bf r}, \theta))$ \ $\cup$ \\
%&
& $\pi_\kat{$F_s$,\ $F_r$, T,\
  $\lambda_r / \lambda$}
  ({\bf W_\kat{U}}({\bf s}; {\bf r}, \theta))$ \ $\cup$
  \\ [0.5ex]
&
%& $\pi_\kat{$F_r$,\ $F_s$, T,\ and$(\lambda_r,\lambda_s) / \lambda$}
%   (W_{\kat{O}}({\bf s}; {\bf r}, \theta))$ \ $\cup$ \\
%&
& $\pi_\kat{$F_s$,\ $F_r$, T,\
  andNot$(\lambda_r,\lambda_s) / \lambda$}
  ({\bf W_\kat{N}}({\bf s}; {\bf r}, \theta))$
  \\ [0.5ex]
\hline
\end{tabular}
\vspace{0.2cm}
\caption{Definition of TP tuple-based operations}
\label{fig:joinOpsDefinitions}
\end{table}

  \begin{table}[!ht]\centering
  \begin{tabular}{>{\centering\arraybackslash}m{0.6in}
    >{\centering\arraybackslash}m{2.1in}  @{}m{0pt}@{}}
      \hline
      $\textit{\textbf{and}}(\lambda_1,\lambda_2)$ &
      \hspace*{-1in}$~=~ (\lambda_1) \land (\lambda_2)$  &\\ [0.4cm]
      \hline
      $\textit{\textbf{andNot}}(\lambda_1,\lambda_2)$ & $~~=~\left \{ 
          \begin{array}{l l}
             (\lambda_1) & \quad \text{if $\lambda_2 = \mathtt{null}$}\\
             (\lambda_1) \land \neg (\lambda_2) & \quad \text{otherwise}\\
          \end{array} \right.$ &\\[0.8cm]

      \hline
      $\textit{\textbf{or}}(\lambda_1,\lambda_2)$ & $~=~ \left \{ 
          \begin{array}{l l}
            (\lambda_1) & \quad \text{if $\lambda_2 = \mathtt{null}$}\\
            (\lambda_2) & \quad \text{if $\lambda_1 = \mathtt{null}$}\\
            (\lambda_1) \lor (\lambda_2) & \quad \text{otherwise}\\
          \end{array} \right.$ &\\ [1.1cm]
      \hline                 
    \end{tabular}
    \vspace{0.2cm}
      \caption{Definition of lineage-concatenation functions.}
  \label{tab:lineageFunctions}
   \end{table}
\end{definition}


Since each window covers a maximal interval, we guarantee that each 
operation satisfies TP change preservation. Using the appropriate 
lineage-concatenation functions for each window, we guarantee that
the output lineage expressions comply with TP snapshot reducibility. 
The same holds for the output facts since they are the same for each
time point of a window interval and thus of an output interval. 
%For
%every join with negation we include all windows of the positive
%relation with respect to the negative one. The full outer join is 
%symmetric. In this case, the input relations are perceived as both
%positive and thus, the unmatched and negating windows of each
%relation with respect to the other are computed. Due to the 
%symmetricity of the overlapping windows
%(Prop.~\ref{prop:symmetric}), the overlapping windows only need
%to be computed once. 

%\begin{example}
%\end{example}
%
%The result of temporal-probabilistic anti join includes, for
%each time point, the probability that a fact of the left
%relation matches no fact in the right relation under a predicate
%$\theta$. Given $\mathbf{r} \AJoin_{\theta}^\kat{Tp} \mathbf{s}$ %and an output tuple $\tilde{r}$, the non-existence of any tuple
%in the right relation over $\tilde{r}.T$ is required. The TP
%anti join is an operation purely based on negation and thus the
%unmatched and negating windows of ${\bf r}$ based on ${\bf s}$
%are needed for the result. The TP left join includes, at each
%time point, the facts $F_r$ for which there is a non-zero
%probability to be only in ${\bf r}$ and the ones that can be
%matched with a tuple in ${\bf s}$ based on a predicate $\theta$.
%As a result, on top of the unmatched and negating windows, the
%overlapping windows of ${\bf r}$ based on ${\bf s}$ are
%required. Unmatched and negating windows are needed for the
%result, as in the case of the anti join. However, for the
%outer join, not only do we need overlapping windows as well
%but also the attributes of the windows in the above two %categories are differently combined to form output tuples. When
%a tuple $r$ of ${\bf r}$ and a tuple $s$ of ${\bf s}$ overlap at
%a time point $t$, two are the possible outcomes. If both $r$ and
%$s$ are true at $t$ and the predicate $\theta$ is satisfied, the
%two tuples can be combined to produce an output tuple with fact
%$(r.F,s.F)$. Otherwise, if $r$ is true but all the tuples in
%${\bf s}$ with which it could have been combined are false, an
%output tuple with fact $(r.F,\mathtt{null})$ would be formed.
%These two potential tuples are produced by an overlapping and a
%negating lineage-enhanced temporal windows respectively. 


%In TP databases, the result of a \emph{TP left outer join}
%includes, at each time point, contains all facts of the "left"
%relation, even if the join-condition does match them with a fact
%in the "right" relation.
